Simulating Human Gaze with Neural Visual Attention

Existing models of human visual attention are generally unable to incorporate direct task guidance and therefore cannot model an intent or goal when exploring a scene. To integrate guidance of any downstream visual task into attention modeling, we propose the Neural Visual Attention (NeVA) algorithm. To this end, we impose to neural networks the biological constraint of foveated vision and train an attention mechanism to generate visual explorations that maximize the performance with respect to the downstream task. We observe that biologically constrained neural networks generate human-like scanpaths without being trained for this objective. Extensive experiments on three common benchmark datasets show that our method outperforms state-of-the-art unsupervised human attention models in generating human-like scanpaths.

==> imgs/tex_images/NeVA.tex <==
\definecolor{darkmidnightblue}{rgb}{0.0, 0.2, 0.4}


\begin{tikzpicture}[
squarednode/.style={rectangle, draw=darkmidnightblue, fill=white, very thick, minimum size=10mm},
]

\newcommand\wa{1.5cm}


\newcommand\xa{0}
\newcommand\xb{3}
\newcommand\xc{5.5}
\newcommand\xd{8}
\newcommand\xe{10.5}
\newcommand\xf{13.5}
\newcommand\xg{16.5}

\newcommand\ya{-2.1}
\newcommand\yb{2.5}

\newcommand\xla{10.5}
\newcommand\xlb{11.0}

\newcommand\yla{3.0}
\newcommand\ylb{2.5}
\newcommand\ylc{2.0}



%Information Processing
%Error Propagation
%Sampling

% ----------------- Legend --------------------

\draw[->,thick,black] (\xla,\yla) -- (\xlb,\yla) node[anchor=west] {Signal propagation};

\draw[->,thick,black,dashed] (\xla,\ylb) -- (\xlb,\ylb) node[anchor=west] {Loss propagation};

\draw[->,thick,black,dotted] (\xla,\ylc) -- (\xlb,\ylc) node[anchor=west] {Stimulus sampling};

% ----------------- Nodes --------------------

%Current Attention Model
\node[squarednode, label=above:{Attention\textsubscript{t=2}}] (CurrentAttention) at (\xb,0)
    {\includegraphics[width=\wa]{imgs/png_imgs/Attention_1.png}};
    
%Foveation Model
\node[squarednode] (FoveationMechanism) at (\xc,0) {$\pi$};

%Stimulus
\node[squarednode, label=above:{Stimulus}] (Stimulus) at (\xc,\yb)
    {\includegraphics[width=\wa]{imgs/png_imgs/Stimulus.png}};

%Perceived 2
\node[squarednode, label=above:{Perceived\textsubscript{t=2}}] (Perceived) at (\xd,0)
    {\includegraphics[width=\wa]{imgs/png_imgs/Perceived_1.png}};
    
%Foveation Model
\node[squarednode] (HiddenState) at (\xe,0) {$h_{t=2}$};

%Task  Model
\node[squarednode] (TaskModel) at (\xg,\ya) {$\tau$};

%Internal Representation
% \node[squarednode,label=below:{Internal Representation}] (InternalRepresentation) at (\xe, \ya){%
%     \begin{tabular}[b]{@{}c@{}}
%       \raisebox{-\dp11}{\includegraphics[width=\wa]{imgs/png_imgs/Attention_Total.png}}
%       \raisebox{-\dp11}{{\includegraphics[width=\wa]{imgs/png_imgs/Internal.png}}}
%     \end{tabular}%
% };

\node[squarednode] (CumAttention) at (\xf, 0)
    {\includegraphics[width=\wa]{imgs/png_imgs/Attention_Total.png}};


\node[squarednode,label=below:{Agent State}] (AgentState) at (\xf, \ya)
    {\includegraphics[width=\wa]{imgs/png_imgs/Internal.png}};



%Attention Model
\node[squarednode] (AttentionModel) at (\xb,\ya) {$\alpha$};

%Perceived 1
\node[squarednode, label=above:{Perceived\textsubscript{t=1}}] (InitalPerceived) at (\xd,\yb)
    {\includegraphics[width=\wa]{imgs/png_imgs/Perceived_0.png}};

% ------------------ Arrows -------------------

\draw[->] (CurrentAttention.15)  -- (FoveationMechanism.155);
\draw[->,dashed] (FoveationMechanism.205)  -- (CurrentAttention.345);

\draw[->] (FoveationMechanism.25)  -- (Perceived.165);
\draw[->, dashed] (Perceived.195)  -- (FoveationMechanism.335);

\draw[->, thick, dotted] (Stimulus.south)  -- (FoveationMechanism.north);

\draw[->] (Perceived.15)  -- (HiddenState.155);
\draw[->, dashed] (HiddenState.205)  -- (Perceived.345);

\draw[->] (HiddenState.25) -- node[above] {aggregate} (CumAttention.165);
\draw[->, dashed] (CumAttention.195)  -- (HiddenState.335);

\draw[->] (CumAttention.285)  -- (AgentState.75);
\draw[->, dashed] (AgentState.105)  -- (CumAttention.255);

\draw[->] (AgentState.15)  -- (TaskModel.155);
\draw[->, dashed] (TaskModel.205)  -- (AgentState.345);
\draw[->] (AgentState.west)  -- (AttentionModel.east);

\draw[->] (AttentionModel.115)  -- (CurrentAttention.255);
\draw[->,dashed] (CurrentAttention.285)  -- (AttentionModel.65);


\end{tikzpicture}





% \begin{tikzpicture}[
% squarednode/.style={rectangle, draw=darkmidnightblue, fill=white, very thick, minimum size=10mm},
% ]

% \newcommand\wa{1.5cm}


% \newcommand\xa{0}
% \newcommand\xb{3}
% \newcommand\xc{5.5}
% \newcommand\xd{8}
% \newcommand\xe{10.5}
% \newcommand\xf{13.5}

% \newcommand\ya{-2.1}
% \newcommand\yb{2.5}

% \newcommand\xla{10.5}
% \newcommand\xlb{11.0}

% \newcommand\yla{3.0}
% \newcommand\ylb{2.5}
% \newcommand\ylc{2.0}



% %Information Processing
% %Error Propagation
% %Sampling

% % ----------------- Legend --------------------

% \draw[->,thick,black] (\xla,\yla) -- (\xlb,\yla) node[anchor=west] {Signal propagation};

% \draw[->,thick,black,dashed] (\xla,\ylb) -- (\xlb,\ylb) node[anchor=west] {Loss propagation};

% \draw[->,thick,black,dotted] (\xla,\ylc) -- (\xlb,\ylc) node[anchor=west] {Stimulus sampling};

% % ----------------- Nodes --------------------

% %Current Attention Model
% \node[squarednode, label=above:{Attention\textsubscript{t=2}}] (CurrentAttention) at (\xb,0)
%     {\includegraphics[width=\wa]{imgs/png_imgs/Attention_1.png}};
    
% %Foveation Model
% \node[squarednode] (FoveationMechanism) at (\xc,0) {$\pi$};

% %Stimulus
% \node[squarednode, label=above:{Stimulus}] (Stimulus) at (\xc,\yb)
%     {\includegraphics[width=\wa]{imgs/png_imgs/Stimulus.png}};

% %Perceived 2
% \node[squarednode, label=above:{Perceived\textsubscript{t=2}}] (Perceived) at (\xd,0)
%     {\includegraphics[width=\wa]{imgs/png_imgs/Perceived_1.png}};
    
% %Foveation Model
% \node[squarednode] (HiddenState) at (\xe,0) {$h_{t=2}$};

% %Task  Model
% \node[squarednode] (TaskModel) at (\xf,\ya) {$\tau$};

% %Internal Representation
% \node[squarednode,label=below:{Internal Representation}] (InternalRepresentation) at (\xe, \ya){%
%     \begin{tabular}[b]{@{}c@{}}
%       \raisebox{-\dp11}{\includegraphics[width=\wa]{imgs/png_imgs/Attention_Total.png}}
%       \raisebox{-\dp11}{{\includegraphics[width=\wa]{imgs/png_imgs/Internal.png}}}
%     \end{tabular}%
% };

% %Attention Model
% \node[squarednode] (AttentionModel) at (\xb,\ya) {$\alpha$};

% %Perceived 1
% \node[squarednode, label=above:{Perceived\textsubscript{t=1}}] (InitalPerceived) at (\xd,\yb)
%     {\includegraphics[width=\wa]{imgs/png_imgs/Perceived_0.png}};

% % ------------------ Arrows -------------------

% \draw[->] (CurrentAttention.15)  -- (FoveationMechanism.155);
% \draw[->,dashed] (FoveationMechanism.205)  -- (CurrentAttention.345);

% \draw[->] (FoveationMechanism.25)  -- (Perceived.165);
% \draw[->, dashed] (Perceived.195)  -- (FoveationMechanism.335);

% \draw[->, thick, dotted] (Stimulus.south)  -- (FoveationMechanism.north);

% \draw[->] (Perceived.15)  -- (HiddenState.155);
% \draw[->, dashed] (HiddenState.205)  -- (Perceived.345);

% \draw[->] (HiddenState.295)  -- (InternalRepresentation.74);
% \draw[->, dashed] (InternalRepresentation.105)  -- (HiddenState.245);

% \draw[->] (InternalRepresentation.10)  -- (TaskModel.150);
% \draw[->, dashed] (TaskModel.210)  -- (InternalRepresentation.350);
% \draw[->] (InternalRepresentation.west)  -- (AttentionModel.east);

% \draw[->] (AttentionModel.115)  -- (CurrentAttention.255);
% \draw[->,dashed] (CurrentAttention.285)  -- (AttentionModel.65);


% \end{tikzpicture}

